StarNet: Targeted Computation for Object Detection in Point Clouds

Detecting objects from LiDAR point clouds is an important component of self-driving car technology as LiDAR provides high resolution spatial information. Previous work on point-cloud 3D object detection has re-purposed convolutional approaches from traditional camera imagery. In this work, we present an object detection system called StarNet designed specifically to take advantage of the sparse and 3D nature of point cloud data. StarNet is entirely point-based, uses no global information, has data dependent anchors, and uses sampling instead of learned region proposals. We demonstrate how this design leads to competitive or superior performance on the large Waymo Open Dataset and the KITTI detection dataset, as compared to convolutional baselines. In particular, we show how our detector can outperform a competitive baseline on Pedestrian detection on the Waymo Open Dataset by more than 7 absolute mAP while being more computationally efficient. We show how our redesign---namely using only local information and using sampling instead of learned proposals---leads to a significantly more flexible and adaptable system: we demonstrate how we can vary the computational cost of a single trained StarNet without retraining, and how we can target proposals towards areas of interest with priors and heuristics. Finally, we show how our design allows for incorporating temporal context by using detections from previous frames to target computation of the detector, which leads to further improvements in performance without additional computational cost.

==> sections/algorithm.tex <==
\begin{figure}
\begin{minipage}{0.5\textwidth}

    \begin{algorithm*}[H]
        \footnotesize
        \caption{\name}
        \label{alg:starnet}
        
        \SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        
        \Input{$N, K, R, G, X=\{\vec{x}_i\}, F=\{\vec{f}_i\}, A=\{anchors\}$, where $|A|=G^2$}
        \Output{Coordinates and scores of boxes $B$}
        
          // Samples $N$  centers from $X$.
          
          $ C \longleftarrow Sample(X, N)$
          
          $ B \longleftarrow \emptyset$
          
          \For{$i \in C$} {
          
            // Samples K points near $\vec{x}_i$. 
            
            $P = Neighbor(\vec{x}_i, K, R)$
            
            // Featurizes points around $\vec{x}_i$.
            
            $\vec{u} = Featurize(\{\vec{x}_j|j \in P\}, \{\vec{f}_j|j \in P\})$
            
            // Predicts boxes and their scores, given 
            
            // feature $\vec{u}$ and anchors $A$.
            
            $B' = PredictBoxes(\vec{u}, A)$\
              
            $B \longleftarrow B \cup B'$
        }
          
        $ B \longleftarrow NonMaximumSuppression(B)$

    \end{algorithm*}

\end{minipage}
\label{fig:algorithm}
\end{figure}


==> sections/data_aug_table_2.tex <==

\begin{table*}[th!]
\footnotesize
\begin{center}
\bgroup
\def\arraystretch{1.4}%
\begin{tabular}{| l || c | c | c || c | c | c || c | c | c |}
\hline
& \multicolumn{3}{|c||}{Car}		& \multicolumn{3}{|c||}{Pedestrian}		& \multicolumn{3}{|c|}{Cyclist}	\\ \hline
					& Easy		& Mod.		& Hard		& Easy		& Mod.		& Hard		& Easy		& Mod.		& Hard	\\ \hline 
\hline
no augmentations & 77.8		& 68.2  & 65.7	  & 45.5	& 40.8			& 36.9		& 56.1 		& 36.9		& 35.5	\\
+ global augment	& 85.4		& 74.8	& 72.7   & 46.3	& 39.4			& 36.2		& 75.8 		& 51.9		& 48.7	\\
+ bbox augment	& 86.6		& 77.0	& 74.6   & 63.9	& 56.5			& 52.4		& 81.5 		& 	58.3	& 54.8	\\
+ both	& 90.4		& 79.7	& 77.7   & 71.8	& 61.0			& 53.8		& 86.5 		& 65.2		& 66.0	\\
\hline
\end{tabular}
\egroup
\end{center}
\vspace{0.1cm}
\caption{\textbf{Data augmentation improves performance substantially on KITTI.} All results reported on 3D detection metric for {\it validation} data. Global data augmentations consist of randomly flipping about $y$-axis, uniformly randomly rotating all points $\pm\,45^\circ$, uniformly randomly scaling all points $[0.95, 1.05]$ and randomly translating individual points along the $z$-axis with std of 0.35. Bounding box augmentations consist of augmenting the bounding boxes from a ground truth data base ($< 25$ boxes per scene) \cite{yan2018second} and uniformly randomly rotating boxes by $\pm \,9^\circ$.}
\label{table:augmentation-studies}
\end{table*}
